Evasive Hardware Trojan through Adversarial Power Trace

The globalization of the Integrated Circuit (IC) supply chain, driven by time-to-market and cost considerations, has made ICs vulnerable to hardware Trojans (HTs). Against this threat, a promising approach is to use Machine Learning (ML)-based side-channel analysis, which has the advantage of being a non-intrusive method, along with efficiently detecting HTs under golden chip-free settings. In this paper, we question the trustworthiness of ML-based HT detection via side-channel analysis. We introduce a HT obfuscation (HTO) approach to allow HTs to bypass this detection method. Rather than theoretically misleading the model by simulated adversarial traces, a key aspect of our approach is the design and implementation of adversarial noise as part of the circuitry, alongside the HT. We detail HTO methodologies for ASICs and FPGAs, and evaluate our approach using TrustHub benchmark. Interestingly, we found that HTO can be implemented with only a single transistor for ASIC designs to generate adversarial power traces that can fool the defense with 100% efficiency. We also efficiently implemented our approach on a Spartan 6 Xilinx FPGA using 2 different variants: (i) DSP slices-based, and (ii) ring-oscillator-based design. Additionally, we assess the efficiency of countermeasures like spectral domain analysis, and we show that an adaptive attacker can still design evasive HTOs by constraining the design with a spectral noise budget. In addition, while adversarial training (AT) offers higher protection against evasive HTs, AT models suffer from a considerable utility loss, potentially rendering them unsuitable for such security application. We believe this research represents a significant step in understanding and exploiting ML vulnerabilities in a hardware security context, and we make all resources and designs openly available online: https://dev.d18uu4lqwhbmka.amplifyapp.com

==> sections/02Background.tex <==

\subsection{Power side-channel based HT detection}

An external characteristic emitted due to the operation of the circuit called side channel information commonly includes power consumption, electromagnetic, and time consumption information. Among side channels that can be exploited from the circuit, power side channel information has been considered an effective method to identify HTs during system operation due to its effectiveness, accessibility, and low price. Power side channel detection relies on the fact that the operation of HT deviates the expected power signal. Two requirements should be satisfied for identifying an HT through a power side channel analysis: First, a golden prototype IC for reference side channel signal should be extracted and assuring that the reference chip is not infected. Second, the strength of HT’s power should be high enough to pass the environmental noise and process variation margins. To minimize the requirement mentioned above, some techniques have been proposed in \cite{liu2014hardware, hoque2017golden, faezi2021brain}. These techniques attempt to make side-channel based detection more practical by eliminating the need for acquiring golden ICs and the challenge of inter-die and intra-die process variations.

\begin{comment}
Side-Channel Analysis (SCA) methods especially power analysis, have been considered as more effective methods to identify HTs during system operation. Power analysis attacks exploit the fact that the power consumption of a cryptographic device depends on the data it processes and on the operations it performs \cite{mangard2008power}. We can categorize the power side channel attacks as follow:
\begin{itemize}

    \item \textbf{Simple Power Analysis:} extracts information through direct interpretation of observed power consumption during cryptographic operation.
    
    \item \textbf{Differential Power Analysis:} involves statistically analyzing power consumption measurements from a system.
    
    \item \textbf{High-order Differential power Analysis:} is a method that targets a known or hypothesized relationship between parameters contributing to a side channel 
    
    \item \textbf{Correlation Power Analysis:} are based on the relation between the actual power consumption of a circuit and a power consumption model \eg the Hamming weight model.
    
    \item \textbf{Template Attack:} Records a large number of power traces using many different inputs,  create a template of the circuit's operation and apply this template to victim's small number of power trace record.
 
\end{itemize}
The effectiveness of such methods is based on the size of the Trojan and process variations occurring during the manufacturing process.
\end{comment}

\begin{comment}
Side-Channel Analysis (SCA) methods especially power analysis, have been considered as more effective methods to identify HTs during system operation. The effectiveness of such methods is based on the size of the Trojan and process variations occurring during the manufacturing process. Most publications based on power analysis techniques focus on algorithms to distinguish the power difference caused by HT and methods to augment this difference. The efficacy of these techniques has been evaluated by using \textbf{side-channel sensitivity} in \cite{huang2016mers, lyu2021maxsense, gohil2022attrition}. In this evaluation, the amount of switching caused in a HT-infected design compare with the switching caused in a golden design (\ie HT free). Given $\mathcal{G}$ and \textit{HT} as a golden chip and HT-infected design respectively. The equation \ref{eq:side-channel_sensitivity} represents the side-channel sensitivity of the HT-infected design.

\begin{equation}
\label{eq:side-channel_sensitivity}
    \begin{array}{rlclcl}
        Sensitivity_{HT} = \underset{(u_i, v_i)}{\max}(\frac{switching^{HT}_{(u_i, v_i)} - switching^{\mathcal{G}}_{(u_i, v_i)}}{switching^{\mathcal{G}}_{(u_i, v_i)}} )
        
\end{array}
\end{equation}

Where ($u_i$, $v_i$) denotes $i^{th}$ pair of consecutive test pattern. We use this metric to evaluate the stealthiness of our design optimizations.

\end{comment}



\subsection{Adversarial Attacks on ML }

 Despite their effectiveness and popularity, ML architectures have been shown vulnerable to a critical vulnerability, i.e., adversarial attacks, which jeopardizes their trustworthiness, especially for sensitive domains such as security. Many studies \cite{pgd, fgsm} have shown that CNNs are vulnerable to carefully crafted input noise designed by an adversary to fool them. Very low amplitude perturbations can efficiently force the model to output wrong labels. In the computer vision domain, these adversarial examples are intentionally generated images that look almost exactly the same as the original images but can mislead the classifier to provide wrong outputs. Other work \cite{noneed} claimed that adversarial examples are not a practical threat to ML in real-life scenarios. However, physical adversarial attacks have recently been shown to be effective against CNN-based applications in the real-world \cite{phys}.
\noindent 
{\bf Minimizing Injected Noise:} Its essential for the adversary to minimize the added noise to avoid detection.  
%, an adversary, using information learned about the structure of the classifier, tries to craft perturbations added to the input to cause incorrect classification.   In these types of attacks, the adversary desires to minimize this perturbation noise to avoid detection.  
For illustration purposes, consider a CNN used for image classification.  More formally, given an original input image $x$ and a target classification model $ f() ~s.t. ~ f(x) = l $, the problem of generating an adversarial example $x^*$ can be formulated as a constrained optimization \cite{pbform}:

\begin{equation}
\small
\label{eq:adv}
     \begin{array}{rlclcl}
        x^* = \displaystyle \argmin_{x^*}  \mathcal{D}(x,x^*),  
         s.t.  ~ f(x^*) = l^*,  ~ l \neq l^*
\end{array}
\end{equation}


Where $\mathcal{D}$ is the distance metric used to quantify the similarity between two images and the goal of the optimization is to minimize this added noise, typically to avoid detection of the adversarial perturbations. $l$ and $l^*$ are the two labels of $x$ and $x^*$, respectively:  $x^*$ is considered as an adversarial example if and only if the label of the two images are different ($ f(x) \neq  f(x^*) $) and the added noise is bounded ($\mathcal{D}(x,x^*) < \epsilon $ where $\epsilon \geqslant 0 $).

%\noindent
%{\bf Distance Metrics:}
%The adversarial examples and the added perturbations should be visually imperceptible by humans. Since it is hard to model humans' perception, researchers proposed three metrics to approximate humans' perception of visual difference, namely $L_0$, $L_2$, and $L_ \infty$ \cite{C&W}. These metrics are special cases of the $L_p$ norm: 
%\begin{equation}
%    \left\|x\right\|_p = \left( \sum^{n}_{i = 1} \left |x_i \right | ^{p} \right)^{\frac{1}{p}}
%\end{equation}
%These three metrics focus on different aspects of visual significance. $L_0$ counts the number of pixels with different values at corresponding positions in the two images. $L_2$ measures the Euclidean distance between the two images $x$ and $x^*$. $L_ \infty$ measures the maximum difference for all pixels at corresponding positions in the two images.


%The consequences of an adversarial attack can be dramatic.  For example, misclassification of a stop sign as a yield sign or a speed limit sign could lead to material and human damages. Another possible situation is when using CNNs in financial transactions and automatic bank check processing -- using handwritten character recognition algorithms to read digits from bank cheques or using neural networks for amount and signature recognition \cite{cheque}. An attacker could easily fool the model to predict wrong bank account numbers or amount of money or even fake a signature. A dangerous situation, especially with such large sums of money at stake.

